JudgeMix: Judge-Guided Mixed-Rollout Data Synthesis for LLM Agents

Supervised fine-tuning (SFT) on expert trajectories is a standard paradigm for training LLM agents. However, it suffers from a well-known training-inference distribution mismatch, calling for target-aware data synthesis strategies that ground the training data in the target model's native state distribution. To bridge this gap, emerging approaches incorporate the expert either to guide mixed rollouts alongside the target model, or to provide dense step-wise supervision. Nonetheless, existing methods apply expert assistance blind to the target model's inherent behavior: they either disrupt the rollout using sub-optimal random intervention heuristics, or they enforce indiscriminate uniform supervision that unnecessarily overwrites the model's already-correct actions. We introduce JudgeMix, a judge-guided data synthesis framework that dynamically interleaves the target model and expert based on step-wise semantic evaluations. JudgeMix queries expert guidance precisely when the target model struggles, ensuring high trajectory success rates while keeping the state distribution aligned with the target model. It additionally uses the judge evaluation to reweight expert supervision on different steps, preserving model's inherent valid behavior while correcting its errors. On two agentic tool-use benchmarks, AppWorld and AutomationBench, JudgeMix demonstrates consistent superior performance to existing methods, with improvements up to 10 pass@1 points.

==> tables/ablation_weighted_supervision.tex <==
\begin{table}[t]
    \caption{Ablation study on the effect of weighted supervision as $w$ varies in \cref{eq:supervision_weight}. We report performance on AppWorld with \texttt{Qwen3.5-2B} and \texttt{Qwen3.5-9B} models. We observe that down-weighting supervision signal on targete model's already-success states improves downstream performance.}
    \label{tab:ablation-selective-supervision}
    \centering
    \small
    % \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccc}
        \toprule
        \multirow{4}{*}{\textbf{Method}}
        & \multicolumn{4}{c}{\textbf{AppWorld}} \\
        & \multicolumn{2}{c}{\texttt{Qwen3.5-2B}}
        & \multicolumn{2}{c}{\texttt{Qwen3.5-9B}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & \textbf{Test-N} & \textbf{Test-C}
        & \textbf{Test-N} & \textbf{Test-C} \\
        \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
        & TGC & TGC & TGC & TGC \\
        \midrule
        $w = 1.0$
        & 38.3 & 21.9
        & 77.5 & 66.2 \\
        $w = 0.75$
        & 38.0 & 21.8 
        & 76.2 & 66.6 \\
        $w = 0.5$
        & \textbf{40.9} & \textbf{23.3}
        & 78.5 & 65.9 \\
        $w = 0.25$
        & 39.7 & 22.8 
        & 77.1 & 67.7 \\
        $w = 0$
        & 39.0 & 21.9
        & \textbf{78.7} & \textbf{69.8} \\
        \bottomrule
    \end{tabular}%
    % }
\end{table}
